Proq: Projection-based Runtime Assertions for Debugging on a Quantum Computer

In this paper, we propose Proq, a runtime assertion scheme for testing and debugging quantum programs on a quantum computer. The predicates in Proq are represented by projections (or equivalently, closed subspaces of the state space), following Birkhoff-von Neumann quantum logic. The satisfaction of a projection by a quantum state can be directly checked upon a small number of projective measurements rather than a large number of repeated executions. On the theory side, we rigorously prove that checking projection-based assertions can help locate bugs or statistically assure that the semantic function of the tested program is close to what we expect, for both exact and approximate quantum programs. On the practice side, we consider hardware constraints and introduce several techniques to transform the assertions, making them directly executable on the measurement-restricted quantum computers. We also propose to achieve simplified assertion implementation using local projection technique with soundness guaranteed. We compare Proq with existing quantum program assertions and demonstrate the effectiveness and efficiency of Proq by its applications to assert two ingenious quantum algorithms, the Harrow-Hassidim-Lloyd algorithm and Shor's algorithm.

==> tex/3-Debugging.tex <==
\section{Assertion Design}

The objective of this paper is to provide an approach which the programmers can employ to test their quantum programs on a quantum computer.


In this section, we introduce \myAssertionName, a projection-based assertion scheme.
We first show how to leverage the properties of projective measurement to efficiently check if a state satisfies a projection-based predicate. %, and the reason why the checking procedure is.
Then we formally define the syntax and semantics of a new projection-based $\bf assert $ statement.
Finally, we rigorously prove the feasibility of debugging with projection-based assertions.

\subsection{Checking the satisfactory of a projection-based predicate}

As introduced before, the two key challenges for quantum programming assertions 




A quantum state $\rho$ will not be affected by a projection $P$ if it is in the subspace of $P$.
We can construct a projective measurement $M = \{M_{\bf true}=P,  M_{\bf false}=I-P\}$.
When $\rho$ is in the subspace of $P$, the outcome of this projective measurement is always ``true'' with probability of $1$ and the state is still $\rho$.
Then we can know that $\rho$ satisfies $P$ without changing the state.
When $\rho$ is not in the subspace of $P$, which means that $\rho$ does not satisfy $P$, the probability of outcome ``true'' or ``false'' in the constructed projective measurement is $tr(P\rho)$ or $1-tr(P\rho)$, respectively.
Suppose we perform such procedure $k$ times, the probability that we do not observe any ``false'' outcome is $tr(P\rho)^{k}$. 
Since $tr(P\rho)<1$, this probability approaches 0 very quickly and we can conclude if $\rho$ satisfies $P$ with high certainty within very few executions.

\subsection{Assertion Statement: Syntax and Semantics}

\section{Assertion Design and Implementation}\label{sec:debugging}


In this section, we introduce \myAssertionName, a projection-based assertion scheme.
We first define the syntax and semantics of a new projection-based $\bf assert $ primitive.
Then we introduce several techniques to implement the new $\bf assert $ primitives on measurement-restricted machines.
The proof of all the propositions, lemmas, and theorems in this and the next sections are in Appendix~\ref{appendix:proof}.
%Finally, we prove the robustness of our debugging scheme under small error.

\subsection{Syntax and semantics}
In classical computing, a runtime assertion is checked during execution.
If the program state satisfies the predicate in the assertion, the program will continue with the state unchanged. Otherwise, an exception is raised.
Such property can be achieved with projection based quantum predicates.
%\todo{logical expressive power}

%A quantum state $\rho$ is said to satisfy a projection $P$ when it is in the subspace of $P$.
A quantum state $\rho$ will not be affected by a projection $P$ if it is in the subspace of $P$.
We can construct a projective measurement $M = \{M_{\bf true}=P,  M_{\bf false}=I-P\}$.
When $\rho$ is in the subspace of $P$, the outcome of this projective measurement is always ``true'' with probability of $1$ and the state is still $\rho$.
Then we can know that $\rho$ satisfies $P$ without changing the state.
When $\rho$ is not in the subspace of $P$, which means that $\rho$ does not satisfy $P$, the probability of outcome ``true'' or ``false'' in the constructed projective measurement is $tr(P\rho)$ or $1-tr(P\rho)$, respectively.
Suppose we perform such procedure $k$ times, the probability that we do not observe any ``false'' outcome is $tr(P\rho)^{k}$. 
Since $tr(P\rho)<1$, this probability approaches 0 very quickly and we can conclude if $\rho$ satisfies $P$ with high certainty within very few executions.



%For a runtime assertion, the desired properties are 1) it could 
%\todo{emphasize syntax and semantics}
%3.2.5
%Suggested by \cite{zhou2019applied}, aQHL can be used as a dynamic technique for quantum program debugging, not just for static analysis of quantum programs. To achieve this, we propose a new statement, called ``assertion''.
Thus, quantum runtime assertions can be designed with projections as predicates.
%To enable assertions in a quantum \textbf{while}-language based program, 
We first add a new assertion statement to the quantum \textbf{while}-language grammar.
 
\begin{definition}[\textbf{Syntax} of the assertion statement]
	A quantum assertion is defined as 
	\begin{align*}
	    \ass(\overline{q};P)\equiv P[q_1,...,q_n]
	\end{align*} where $\overline{q}=q_1,...,q_n$ is a collection of quantum variables and $P$ is a projection onto a (closed) subspace of the state space $\cH_{\overline{q}}$.% of $\overline{q}$. 
\end{definition}
\textbf{Semantics of the assertion statement} When executing a assertion statement $\ass(\overline{q};P)$, a constructed projective measurement $M=\{M_{\bf true}=P,M_{\bf false}=I-P\}$ will be performed on the quantum variables  $\overline{q}$.
If the outcome is ``true'', the execution continues. Otherwise an error message is reported and the execution will terminate.

\iffalse
Intuitively, this assertion is used to check whether the state of quantum register $\overline{q}$ falls into a desirable subspace corresponding to $P$. We will often identify projection $P$ with the corresponding subspace. 
In implementation, a projective measurement $M_P = \{M_{\bf true}, M_{\bf false}\}$ is applied to register $\overline{q}$ where $M_{\bf true} = P$ and $M_{\bf false} = I_{\overline{q}}-P$. If the measurement outcome is ``yes'', then execute the rest part of the program; if outcome ``no'' is obtained, 
the program terminates with an error message. This is very similar to the assertions defined in classical programming language.
\fi
%The restriction of $P$ being a projection is desirable.
%{\color{red}desirable, I don't believe necessary; indeed, we can consider non-demolition measurement in our future work.} 
%Considering the meaning of an assertion, we aim to check if the current %state of $\overline{q}$ satisfies $P$, and if it is true we hope the current state is not changed and if not, the program terminate and an error message is alerted. 

\iffalse


%Actually, the restriction of $P$ makes the measurement $M_P$ being a projective measurement, which has a significant advantage in real-world applications: if the current state $\rho$ satisfies $P$, then applying the assertion $\ass(\overline{q};P)$ does not change the current state which ensures that the assertion does not disturb the execution of the program; otherwise, if $\rho$ does not satisfies $P$, there is a certain probability $1-\tr(P\rho)$ to detect this error, and if the error is not detected, $\rho$ is changed to $P\rho P/\tr(P\rho P)$ which satisfies $P$, and this does not affect the following assertions to detect more errors so that at the end, it enable us to detect all possible errors simultaneously.
\fi

With \myAssertionName's runtime assertion defined above, we can inject several assertions in a program since a passed assertion will not affect the state.
And with just a few executions, we can conclude whether the predicates are satisfied with high certainty.
However, we still need to know what predicate $P$ we should use at what place in a program. 

%\myAssertionName~cooperates with aQHL to resolve this problem and is able to derive and inject assertions at arbitrary places in a quantum program.
%Suppose we have a program $S$. We divide the it into $n$ segments $S_1;S_2;\cdots;S_n$ and hope to inject assertion between consecutive program segments. % is a sequential composition of subprograms $S_1,S_2...,S_n$. 
%In \myAssertionName, we first derive a series of Hoare triples $\{P_0\}S_1\{P_1\}$, $\{P_1\}
%S_2\{P_2\}$, $\cdots$,  $\{P_{n-1}\}S_n\{P_n\}$ with aQHL where all $P_{i}$s are projections.
%Then we can define a debugging scheme to check whether $S$ is correct in the sense of Hoare triple $\{P_0\}S\{P_n\}$. 
%\todo{}
%Hoare triples $\{P_0\}S_1\{P_1\}$, $\{P_1\}S_2\{P_2\}$, $\cdots$, $\{P_{n-1}\}S_n\{P_n\}$ to conclude the correctness formula  of $S$.

\begin{definition}
	\label{debuggingscheme}
	A debugging scheme for $S$ is a new program $S^\prime$ with assertions being added between consecutive subprograms $S_i$ and $S_{i+1}$:
	\begin{align*}
	S^\prime\equiv\ %& \ass(\overline{q}_0;P_0); \\
	& S_1; \\
	& \ass(\overline{q}_1;P_1); \\
	& S_2; \\
	& \vdots \\
	& \ass(\overline{q}_{n-1};P_{n-1}); \\
	& S_n; \\
	& \ass(\overline{q}_n;P_{n})
	\end{align*}
	where $\overline{q}_i$ is the collection of quantum variables and $P_i$ is a projection on $\cH_{\overline{q}_i}$ for all $0\le i\le n$.
\end{definition}

The following theorem shows that this debugging scheme is theoretically feasible. 
We first define the distance between two states.
\begin{definition}[Trace distance of states]
    For two states $\rho$ and $\sigma$, the trace distance $D$ between $\rho$ and $\sigma$ is defined as $$D(\rho,\sigma)=\frac{1}{2}tr|\rho-\sigma|$$ where  $tr|X|=tr\sqrt{X^{\dagger}X}$.
\end{definition}


\begin{theorem}[Feasibility of debugging scheme]\label{theorem:feasibility}
Suppose we execute $S^\prime$ for $k$ times with input $\rho$ and collect all the error messages.
\begin{enumerate}
    \item If an error message occurs in $\ass(\overline{q}_m;P_m)$, we conclude that subprogram $S_{m}$ is not correct, i.e., with the input satisfying  precondition $P_{m-1}$, after executing $S_{m}$, the output can violate postcondition $P_m$.
    
    \item If no error message is reported, we claim that program $S$ is close to the bug-free standard program; more precisely, with confidence level $95\%$, 
    \begin{enumerate}
    	\item the confidence interval of $\min_{S_{\rm std}}D\left(\sem{S}(\rho),\sem{S_{\rm std}}(\rho)\right)$ is
    	$\left[0,\frac{0.9n+\sqrt{n}}{\sqrt{k}}\right],$
    	\item the confidence interval of $\min_{S_{\rm std}}F\left(\sem{S}(\rho),\sem{S_{\rm std}}(\rho)\right)$ is
    	$\left[\cos\frac{0.9n+\sqrt{n}}{\sqrt{k}},1\right],$
    \end{enumerate} 
	where the minimum is taken over all bug-free standard program $S_{\rm std}$ that satisfies all assertions with input $\rho$.
    %\item Suppose $S_m$ the first program segment that violates $\{P_{m-1}\}S_m\{P_m\}$, we will get at least one error message with reasonable probability $1-\frac{1}{k}$. 
    %\item Moreover, any error detection does not significantly affect a later detection; that is, even if $S_m$ is wrong, the error detection $S_{m^\prime}$ will still be efficient for all $m^\prime>m$.
\end{enumerate}
Moreover, any error detection does not significantly affect a later detection; that is, in each round, if the test of postcondition of $S_m$ is passed, then the error detection of $S_{m+1}$ is still efficient and effective even if $S_m$ is not correct.
\end{theorem}

\subsection{Transformation techniques for implementation on quantum computers}

Although the debugging scheme is theoretically feasible, the constructed projective measurement may not be directly supported on a realistic quantum computer.
%In aQHL, there is no constraint on the derived projections and the projective measurement in the assertions can be in any basis. % in general. 
The projective measurements derived from the projection-based assertions can be in arbitrary basis.
However, only projective measurements in the computational basis is supported on a realistic quantum computer, which makes the assertions not directly executable on the measurement-restricted quantum computers.
%because usually on po
%the machine constraint makes it difficult to implement a general projective measurement. There is a significant gap between the implementation of all possible  projective measurements and the fact that devices can only achieve measurement for computational basis. 
In this section, we introduce several transformation techniques to %partially
overcome this obstacle. % based on the rank of the projection $P$.

% subsubsection
% 直接通过unitary转化实现：bell state test，先用cnot，然后测量，在转回去
% 拆分顺序测量：
% 引入辅助量子比特：所需空间维数>总维数/2或者分数情形：2qubit，需要3维
% local projection逼近：
% 每一个都引入example
\subsubsection{Additional unitary transformation}
Suppose the assertion $\ass(\overline{q};P)$ we want to implement is over $n$-qubit, that is, $\overline{q} = q_1,q_2,\cdots,q_n$, each of $q_i$ is a single qubit variable. The simplest case is $\rank P = 2^m$ for some  integer $m$ with $0\le m\le n$. % where $\rank P$ is the number of dimensions of the corresponding closed subspace. 
\begin{proposition}\label{prop:unitary}
	For projection $P$ with $\rank P = 2^m$, there exists unitary transformation $U_P$ such that (here $I_{q_i}=I_{\mathcal{H}_{q_{i}}}$):
	$$U_PPU_P^\dag = Q_{q_1}\otimes Q_{q_2}\otimes\cdots\otimes Q_{q_n}=\bigotimes_{i=1}^nQ_{q_i}\triangleq Q_P,$$
	where $Q_{q_i}$ is either $\qbit{0}{q_i}$, $\qbit{1}{q_i}$ or $I_{q_i}$  for each $1\le i\le n$.
\end{proposition}


We call the pair $(U_P,Q_P)$ an \textbf{i}mplementation in \textbf{c}omputati-onal \textbf{b}asis (ICB for short) of $\ass(\overline{q};P)$.
Generally, ICB is not unique. 
According to this proposition, we have the following procedure to implement ${\bf assert}(\overline{q};P)$:
\begin{enumerate}
	\item Apply $U_P$ on $\overline{q}$;
	\item Check $Q_P$ in the following steps:
	For each $1\le i\le n$, if $Q_{q_i} = \qbit{0}{q_i}$ or $\qbit{1}{q_i}$, then measure $q_i$ in the computational basis to see whether the outcome $k$ is consistent with $Q_{q_i}$; that is, $Q_{q_i} = \qbit{k}{q_i}$. If all outcomes are consistent, go ahead; otherwise, we terminate the program with an error message;
	\item Apply $U_P^\dag$ on $\overline{q}$.
\end{enumerate}

\begin{example}
	Given a two-qubit register $\overline{q} = q_1,q_2$, if we want to test whether it is in the Bell state (maximally entangled state) $|\Phi\> = \frac{1}{\sqrt{2}}(|00\>+|11\>)$, we can use the assertion ${\bf assert}(\overline{q}; P = |\Phi\>\<\Phi|)$.
	To implement it in the computational basis, noting that 
	\begin{align*}
	     & {\rm CNOT}[q_1,q_2]H[q_1]\cdot P\cdot H[q_1]{\rm CNOT}[q_1,q_2]  = \qbit{0}{q_1}\otimes \qbit{0}{q_2}
	\end{align*}
%$${\rm CNOT}[q_1,q_2]H[q_1]\cdot P\cdot H[q_1]{\rm CNOT}[q_1,q_2] = \qbit{0}{q_1}\otimes \qbit{0}{q_2}$$ 
we can first apply ${\rm CNOT}$ gate on $\overline{q}$ and $H$ gate on $q_1$, then measure $q_1$ and $q_2$ in the computational basis. If both outcomes are ``0'', we apply $H$ on $q_1$ and ${\rm CNOT}$ on $\overline{q}$ again to recover the state; otherwise, we terminate the program and report that the state is {\rm not} Bell state $|\Phi\>$. 
\end{example}

\subsubsection{Combining assertions}

%{\color{red}I guess,  we should expand the assertion language to include
%$\bigwedge_i A_i, \bigvee_i A_i$, interpreted as $\bigcap_i, \bigoplus_i$ %(direct sum); exactly connectives in Birkhoff-von Neumann Quantum logic} 

The method introduced above only applies to the case that $\rank P = 2^m$ with some integer $m$. The following proposition provides us a way for dealing with the more general case $\rank P\le 2^{n-1}$: split the assertion into multiple sub-assertions that satisfy the above conditions.% For simplicity, we will identify a projection operator with the corresponding subspace.  

\begin{proposition}\label{prop:combining}
	For projection $P$ with $\rank P \le 2^{n-1}$, there exist projections $P_1,P_2,\cdots,P_l$ satisfying $\rank P_i = 2^{n_i}$ for all $1\le i\le l$, such that 
	$P = P_1\cap P_2\cap\cdots\cap P_l.$
\end{proposition}

Essentially, this way works for our scheme because conjunction can be defined in Birkhoff-von Neumann quantum logic.  
Theoretically, $l=2$ is sufficient; but in practice a larger $l$ allows us to choose simpler $P_i$ for each $i\leq l$.   

%{\color{red} How about use $\bigvee_i$?
%$$\rank P= 2^{i_1}+2^{i_2}+...+2^{i_l}$$ with $0\leq i_1<i_2<...<i_l\leq n-1.$}

Using the above proposition, to implement $\ass(\overline{q};P)$, we may sequentially apply $\ass(\overline{q};P_1)$, $\ass(\overline{q};P_2),\ \cdots$
, $\ass(\overline{q};P_l)$. Suppose $(U_{P_i}, Q_{P_i})$ is an ICB of $\ass(\overline{q};P_i)$ for $1\le i\le l$, we have the following  scheme to implement $\ass(\overline{q};P)$:
\begin{enumerate}
	\item Set counter $i = 1$;
	\item If $i=1$, apply $U_{P_1}$; else if $i=l$, apply $U_{P_l}^\dag$ and return; otherwise, apply $U_{P_{i-1}}^\dag U_{P_{i}}$;
	\item Check $Q_{P_i}$; $i:=i+1$; go to step $2$.
\end{enumerate}


\begin{example}
	Given register $\overline{q} = q_1,q_2,q_3$, how to implement $\ass(\overline{q};P)$ where 
	$P = \qbit{00}{q_1q_2}\otimes I_{q_3} + \qbit{111}{q_1q_2q_3}?$
	
	Observe that $P = P_1 \cap P_2$ where
	\begin{align*}
		&P_1 = (\qbit{00}{q_1q_2} + \qbit{11}{q_1q_2})\otimes I_{q_3}, \\
		&P_2 = \qbit{00}{q_1q_2}\otimes I_{q_3} + \qbit{100}{q_1q_2q_3}+\qbit{111}{q_1q_2q_3}.
	\end{align*}		
	with following properties:
	\begin{align*}
		&{\rm CNOT}[q_1,q_2]\cdot P_1\cdot {\rm CNOT}[q_1,q_2] = I_{q_1}\otimes\qbit{0}{q_2}\otimes I_{q_3} \\
		&{\rm Toffoli}[q_1,q_3,q_2]\cdot P_2\cdot {\rm Toffoli}[q_1,q_3,q_2] = I_{q_1}\otimes\qbit{0}{q_2}\otimes I_{q_3}.
	\end{align*}
	Therefore, we are able to implement $\ass(\overline{q};P)$ by:
	\begin{itemize}
		\item Apply ${\rm CNOT}[q_1,q_2]$;
		\item Measure $q_2$ and check if the outcome is ``0''; if not, terminate and report the error message;
		\item Apply ${\rm CNOT}[q_1,q_2]$ and then ${\rm Toffoli}[q_1,q_3,q_2]$;
		\item Measure $q_2$ and check if the outcome is ``0''; if not, terminate and report the error message;
		\item Apply ${\rm Toffoli}[q_1,q_3,q_2]$.
	\end{itemize}
\end{example}


\subsubsection{Auxiliary qubits}

A case still remains unsolved: $\rank P>2^{n-1}$. To handle this case, the auxiliary qubit is necessary. Without the auxiliary qubit, any measurement divides the entire space into multiple subspaces with dimension at most $2^{n-1}$, which leads to the impossibility of implementing $\ass(\overline{q};P)$. Introducing an auxiliary qubit can solve this difficulty.

Specifically, we introduce an auxiliary qubit $a$ which is initialized to basis state $|0\>$, then implement $$\ass(a,\overline{q};\qbit{0}{a}\otimes P)$$ instead of original $\ass(\overline{q};P)$. Noting that $\rank(\qbit{0}{a}\otimes P) = \rank P\le 2^n$ and the number of qubits is $n+1$ including auxiliary qubit $a$, therefore the methods introduced before is enough to complete the rest steps. Here is a trick to reduce the complexity: we may split $\qbit{0}{a}\otimes P$ with $P_0 = \qbit{0}{a}\otimes I_{\overline{q}}, P_1,\cdots,P_l$ such that $\qbit{0}{a}\otimes P = \bigcap_{i=1}^lP_i$. Since the auxiliary qubit is initialized to $|0\>$, $P_0$ automatically holds and thus we only need to sequentially apply $\ass(a,\overline{q};P_1)$, $\cdots$, $\ass(a,\overline{q};P_l)$. In fact, $l=1$ is enough.

\begin{example}
	Given register $\overline{q}=q_1,q_2$, we aim to implement $\ass(\overline{q};P)$ where
	$P = \qbit{0}{q_1}\otimes I_{q_2} + \qbit{11}{q_1q_2}.$
	
	We may have the decomposition $\qbit{0}{a}\otimes P = P_0\cap P_1$, where	
	\begin{align*}
		&P_0 = \qbit{0}{a}\otimes I_{\overline{q}}, \\
		&P_1 = \qbit{00}{aq_1}\otimes I_{q_2} + \qbit{011}{aq_1q_2}+\qbit{100}{aq_1q_2},
	\end{align*}
	and an ICB of $P_1$ is:
	$${\rm Fredkin}[q_2,a,q_1]\cdot P_1\cdot {\rm Fredkin}[q_2,a,q_1] = I_{a}\otimes\qbit{0}{q_1}\otimes I_{q_2}.$$
	
	Note that $P_0$ automatically holds since the auxiliary qubit $a$ is in $|0\>$, we only need to execute:
	\begin{itemize}
		\item Introduce auxiliary qubit $a$, initialize it to $|0\>$;
		\item Apply ${\rm Fredkin}[q_2,a,q_1]$;
		\item Measure $q_1$ and check if the outcome is ``0''; if not, terminate and report the error message;
		\item Apply ${\rm Fredkin}[q_2,a,q_1]$; free the auxiliary qubit $a$.
	\end{itemize}
\end{example}



==> tex/4-EfficientProjection.tex <==
\section{Efficiency and Robustness of Debugging}\label{sec:efficiency}
In this section, we discuss efficient assertion designs and the decomposition of the introduced unitary transformation. We also prove the robustness of our debugging scheme. In other words, the accumulated error from the assertions is bounded when the error from each assertion is small.

\subsection{Local projection: trade-off between efficiency and effectiveness}
\label{sec:efficient-implementation}
% maybe another paper
% some small projection operators
%It is very common that the projective measurement $P$ we want to implement is very hard to implement. Therefore, rather than implement $P$, we can implement a class of projective measurements $Q_1,Q_2,\cdots, Q_m$ with $Q_i\geq P$ for any $i$.

For projections over multiple qubits, it is quite common to be highly entangled, which leads to the difficulty of implementing the unitary transformation in ICB.
It is possible to slightly relax the constraints in the predicates for simplified assertion implementation. % by slightly loosing the constraints in the predicates.
To achieve this trade-off, we employ a commonly used approach in quantum information science, namely the quantum state tomography via local measurements~\cite{PhysRevLett.89.207901,PhysRevA.86.022339,PhysRevLett.118.020401}.
%To partially overcome this obstacle, we employ a commonly used approach in quantum information science, namely the quantum state tomography via local measurements  \cite{PhysRevLett.89.207901,PhysRevA.86.022339,PhysRevLett.118.020401}.

We first introduce the notion of partial trace to describe the state (operator) of a subsystem. 
Let $\overline{q}_1$ and $\overline{q}_2$ be two disjoint registers with corresponding state Hilbert space $\cH_{\overline{q}_1}$ and $\cH_{\overline{q}_2}$, respectively. 
The partial trace over $\cH_{\overline{q}_1}$ is a mapping $\tr_{\overline{q}_1}(\cdot)$ from operators on $\cH_{\overline{q}_1}\otimes\cH_{\overline{q}_2}$ to operators in $\cH_{\overline{q}_2}$ defined by:
$\tr_{\overline{q}_1}(|\phi_1\>_{\overline{q}_1}\<\psi_1|\otimes|\phi_2\>_{\overline{q}_2}\<\psi_2|) = \<\psi_1|\phi_1\>\cdot|\phi_2\>_{\overline{q}_2}\<\psi_2|$ for all $|\phi_1\>,|\psi_1\>\in\cH_{\overline{q}_1}$ and $|\phi_2\>,|\psi_2\>\in\cH_{\overline{q}_2}$ together with linearity.
The partial trace $\tr_{\overline{q}_2}(\cdot)$ over $\cH_{\overline{q}_2}$ can be defined dually. 

To illustrate this idea, we need the following definition of local projection:
%\todo{define partial trace}
\begin{definition}[Local projection]
	Given $\ass(\overline{q};P)$, a local projection $P_{\overline{q}^\prime}$ over $\overline{q}^\prime\subseteq\overline{q}$ is defined as:
	$$P_{\overline{q}^\prime} = \supp\left(\tr_{\overline{q}\backslash\overline{q}^\prime}(P)\right).$$
\end{definition}
Realizing that $P\subseteq P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$, the implementation of $\ass(\overline{q}^\prime;P_{\overline{q}^\prime})$ can partially test whether the state satisfies $P$. Moreover, if the number of qubits of $\overline{q}^\prime$ is small, the implementation of  $\ass(\overline{q}^\prime;P_{\overline{q}^\prime})$ can be efficiently achieved.
Therefore, we have the following implementation strategy which is essentially a trade-off between checking efficiency and effectiveness:
\begin{itemize}
	\item Find a sequence of local projection $P_{\overline{q}_1}, P_{\overline{q}_2},\cdots,P_{\overline{q}_l}$ of $\ass(\overline{q};P)$;
	\item Instead of implementing the original $\ass(\overline{q};P)$, we sequentially apply $\ass(\overline{q}_1;P_{\overline{q}_1})$, $\ass(\overline{q}_2;P_{\overline{q}_2})$, $\cdots$, $\ass(\overline{q}_2;P_{\overline{q}_l})$.
\end{itemize}
% maybe another paper
% some small projection operators
%It is very common that the projective measurement $P$ we want to implement is very hard to implement. Therefore, rather than implement $P$, we can implement a class of projective measurements $Q_1,Q_2,\cdots, Q_m$ with $Q_i\geq P$ for any $i$.

% We illustrate our idea in the following example. 
% Suppose we want to implement $P=\op{\psi}{\psi}$ where $\ket{\psi}$ is a highly entangled $n$-qubit state. 
% Now we can implement measurements $Q_{i,j}$ where $Q_{i,j}=\supp(\psi_{i,j})$ with $\psi_{i,j}$ be the reduced density matrix on qubit $i,j$ for quantum state $\ket{\psi}$.

%\iffalse
%This idea has deep connection to the quantum marginal problem. Understanding the relation between quantum marginals is considered to be one of the most fundamental problems in quantum information theory and quantum chemistry because many important physical quantities, such as energy and entropy, only depend on very
%small parts of a whole system only--these small parts are the marginal or reduced density matrices. A great deal of effort has been devoted to understanding this problem, even in the case of low dimension or a small number
%of parties. Many quantum states are uniquely determined by the support of 
%their local reduced density matrices \cite{PhysRevLett.118.020401}, which would make this idea stronger than it looks like.

%Here we can formulate the condition as follows, $\ket{\psi}$ is uniquely determined by the support of its local reduced density matrices if and only if the frustration-free Hamiltonian
%$$
%H=\sum_{i,j }I_{[n]\{i,j}\otimes Q_{i,j}
%$$
%has a unit ground state.

% Surely, other projective local measurements can also be used for approximately implementing a desire entangled projective measurement.
% \todo{pending Li's example}
% \todo{section 3.3 needs rephrase, too many new terms....}

%Let us consider a more complicated example to see how it works.
\begin{example}
Given register $\overline{q} = q_1,q_2,q_3,q_4$, we want to check if the state is the superposition of following states:
\begin{align*}
&|\psi_1\> = |+\>_{q_1}|111\>_{q_2q_3q_4},\quad |\psi_2\> = |000\>_{q_1q_2q_3}|-\>_{q_4},\\
&|\psi_3\> = \frac{1}{\sqrt{2}}|0\>_{q_1}\left(|00\>_{q_2q_3}+|11\>_{q_2q_3}\right)|1\>_{q_4}.
\end{align*}
To accomplish this, we may apply the assertion $\ass(\overline{q};P)$ with $P = \supp\left(\sum_{i=1}^3|\psi_i\>\<\psi_i|\right)$. However, projection $P$ is highly entangled which prevents efficient implementation. 
Observe the following local projections:
\begin{align*}
P_{q_1q_2} &= \tr_{q_3q_4}(P) = \qbit{0}{q_1}\otimes I_{q_2} + \qbit{11}{q_1q_2},\\
P_{q_2q_3} &= \tr_{q_1q_4}(P) = \qbit{00}{q_2q_3} + \qbit{11}{q_2q_3},\\
P_{q_3q_4} &= \tr_{q_1q_2}(P) = \qbit{00}{q_3q_4} + \qbit{11}{q_3q_4}.
\end{align*}
To avoid implementing $\ass(\overline{q},P)$ directly, we may apply $\ass(q_1,q_2; ~P_{q_1q_2})$, $\ass(q_2,q_3; ~P_{q_2q_3})$, and $\ass(q_3,q_4; \\P_{q_3q_4})$ instead. Though these assertions do not fully characterize the required property, their implementation requires only relatively low cost, i.e., each of them only acts on two qubits.
\end{example}

\subsection{Unitary transformation decomposition}
%optimization: cost 
%不同模型下的cost T count, Cnot count,...
%The additional unitary transformation is essential in \myAssertionName. 
The additional unitary transformation, which is essential in \myAssertionName, is usually decomposed into a directly supported gate set when being implemented on a quantum computer.
We focus on assertion scheme design while detailed unitary transformation decomposition is out of the scope of this paper.
Here we only briefly discuss common target gate sets for decomposition, and the metrics to evaluate a %unitary transformation 
decomposition.
%Much like any classical algorithm, a quantum algorithm needs to be implemented efficiently in order to gain maximal possible advantage from executing it.
%A unitary transformation in quantum program is usually broken down into circuits over elementary gates.
It has been proved that arbitrary unitary transformation  can be decomposed into a gate set consisting of CNOT gates and single-qubit gates~\cite{barenco1995elementary}.
CNOT gate count is a commonly used metric due to the high implementation overhead %and error rate 
of a CNOT gate under state-of-the-art technology~\cite{linke2017experimental}.

After considering quantum error correction, the set of the elementary logical gates allowed is dictated by the fault tolerance techniques that limit the efficiency of implementing an arbitrary transformation. 
Recent studies %of fault tolerance techniques 
suggest that the fault-tolerant library should consist of Clifford (single-qubit Pauli, Hadamard, Phase, CNOT gates) and T logical gates, with the understanding that the T gate requires considerably more resources than any of the Clifford gates .
It has become widely accepted that the T-gate count/depth serves as a good first-order approximation of the resource count required to physically implement a quantum circuit \cite{Aliferis:2006:QAT:2011665.2011666, Ross:2016:OAC:3179330.3179331}.

\subsection{Robust debugging scheme}
%ÈçºÎrobust µÄdebug
Similar to the debugging scheme defined in Section~\ref{sec:debugging}, we can still use the projections $P$ and $Q$ appeared in a robust Hoare triple $\{(P,\epsilon)\}S\{(Q,\delta)\}$~\cite{zhou2019applied} to define the robust debugging scheme for approximate quantum programs while ignoring the parameter $\epsilon$ and $\delta$. 
However, it is worthwhile to show this robust debugging scheme is still correct and efficient to detect possible errors of the program when $\epsilon$ and $\delta$ is small.

%We first introduce the well-known gentle measurement lemma \cite{Winter99}:
We first study a special case of the gentle measurement lemma~\cite{Winter99} with projections.
The result is slightly stronger than the original one in \cite{Winter99} under the constraint of projection.

%\textbf{Define Distance, Remove the proof to appendix}
%\begin{definition}[Trace distance of states]
%    For two states $\rho$ and $\sigma$, the trace distance $D$ between $\rho$ and $\sigma$ is defined as $$D(\rho,\sigma)=\frac{1}{2}tr|\rho-\sigma|.$$
%\end{definition}
\begin{lemma}[Gentle measurement with projections]\label{lemma:gentle}
	For projection $P$ and density operator $\rho$, if $\tr(P\rho)\ge1-\epsilon$, then	
	\begin{enumerate}
		\item $D\Big(\rho,\frac{P\rho P}{\tr(P\rho P)}\Big)\le\epsilon+\sqrt{\epsilon(1-\epsilon)}.$
		\item $F\Big(\rho,\frac{P\rho P}{\tr(P\rho P)}\Big)\ge\sqrt{1-\epsilon}.$
	\end{enumerate}
\end{lemma}
% \begin{proof}
% 	For pure state $|\psi\>$, we have:
% 	\begin{align*}
% 	\tr|P|\psi\>\<\psi| P^\perp| &= \tr\sqrt{P|\psi\>\<\psi| P^\perp P^\perp|\psi\>\<\psi|P} \\
% 	&=\sqrt{\<\psi| P^\perp P^\perp|\psi\>}\tr\sqrt{P|\psi\>\<\psi|P} \\
% 	&= \sqrt{\<\psi| P^\perp |\psi\>}\sqrt{\<\psi|P|\psi\>} \\
% 	&= \sqrt{\tr(P|\psi\>\<\psi|)}\sqrt{\tr(P^\perp|\psi\>\<\psi|)}.
% 	\end{align*}
% 	Therefore, for any density operators $\rho$ with spectral decomposition $\rho = \sum_ip_i|\psi_i\>\<\psi_i|$, we have:
% 	\begin{align*}
% 	\tr|P\rho P^\perp| &= \tr|P\sum_ip_i|\psi_i\>\<\psi_i| P^\perp| \\
% 	&\le \sum_ip_i\tr|P|\psi_i\>\<\psi_i| P^\perp| \\
% 	&= \sum_i\sqrt{p_i\tr(P|\psi_i\>\<\psi_i|)}\sqrt{p_i\tr(P^\perp|\psi_i\>\<\psi_i|)} \\
% 	&\le \sqrt{\sum_ip_i\tr(P|\psi_i\>\<\psi_i|)}\sqrt{\sum_ip_i\tr(P^\perp|\psi_i\>\<\psi_i|)} \\
% 	&= \sqrt{\tr(P\rho)\tr(P^{\perp}\rho)}
% 	\end{align*}
% 	using the Cauchy-Schwarz inequality. Now, it is straightforward to have:
% 	\begin{align*}
% 	&D\Big(\rho,\frac{P\rho P}{\tr(P\rho P)}\Big) \\
% 	=\ & \frac{1}{2}\tr\Big|P\rho P+P^\perp \rho P+P\rho P^\perp+P^\perp \rho P^\perp - \frac{P\rho P}{\tr(P\rho P)}\Big| \\
% 	\le\ & \frac{1}{2}\tr|P\rho P|\Big|1-\frac{1}{\tr(P\rho P)}\Big| + \frac{1}{2}|P\rho P^{\perp}+P^{\perp}\rho P|  \\
% 	&  + \frac{1}{2}|P^{\perp}\rho P^{\perp}|\\
% 	\le\ & \frac{1}{2}(1-\tr(P\rho)) + \tr\big|P\sqrt{\rho}\sqrt{\rho}P^\perp\big| + \frac{1}{2}\tr((I-P)\rho) \\
% 	\le\ & \frac{\epsilon}{2} + \sqrt{\tr(P\rho)\tr(P^{\perp}\rho)} + \frac{\epsilon}{2}\\
% 	\le\ & \epsilon + \sqrt{\epsilon(1-\epsilon)}.
% 	\end{align*}
% 	The restriction of $P$ makes it a slightly stronger than the original one in \cite{Winter99}.
% \end{proof}

Suppose a state $\rho$ satisfies $P$ with error $\epsilon$, 
%a density operator $\rho$ is in $(P,\epsilon)$, 
then $\tr(P\rho)\ge1-\epsilon$ which ensures that, applying the projective measurement $M_P = \{M_{\bf true} = P,\ M_{\bf false} = I-P\}$, we have the outcome ``true'' with probability at least $1-\epsilon$. Moreover, if the outcome is ``true'', the post-measurement state is $\frac{P\rho P}{\tr(P\rho P)}$, which is actually close to the original state $\rho$ in the sense that their trace distance is at most $\epsilon+\sqrt{\epsilon(1-\epsilon)}$.

Consider a program $S = S_1;S_2;\cdots;S_n$ with desired robust Hoare triples $$\{(P_0,\epsilon_0)\}S_1\{(P_1,\epsilon_1)\},\cdots, \{(P_{n-1},\epsilon_{n-1})\}S_n\{(P_n, \epsilon_n)\}$$ which are used to conclude the correctness formula 
$\{(P_0,\epsilon_0)\}\\ S\{(P_n,\epsilon_n)\}$ of $S$. 
The following theorem states that the debugging scheme defined in Definition \ref{debuggingscheme} is still efficient for robust debugging.
\begin{theorem}[Feasibility of robust debugging]\label{theorem:robust}

Assume that all $\epsilon_i$ are small. %, say $\epsilon_i\le\epsilon$. 
Execute $S^\prime$ for $k$ times, and we count $k_m$ for the occurrence of error message for assertion $\ass(\overline{q}_m, P_m)$. 
\begin{enumerate}
    \item If $\frac{k_m}{k-\sum_{i=0}^{m-1}k_i}$ is significantly larger than $\epsilon_m$, we conclude that $S_m$ is not valid for $\{(P_{m-1},\epsilon_{m-1})\}S_m\{(P_m,\epsilon_m)\}$ with high confidence.
    \item If all $\frac{k_m}{k-\sum_{i=0}^{m-1}k_i}$ are close to or smaller than $\epsilon_m$ for all $m\ge1$, we can conclude that %$\{(P_0,\epsilon_0)\}S\{(P_n,\epsilon_n+\delta)\}$ 
    $\{(P_0,0)\}S\{(P_n,\delta)\}$ 
    is valid with high probability, where 
    $\delta = \sum_{i=1}^n\big(\epsilon_i+\sqrt{\epsilon_i(1-\epsilon_i)}\big) \approx \sum_{i=1}^n\sqrt{\epsilon_i}$
    %$\delta = n(\epsilon+\sqrt{\epsilon(1-\epsilon)})\approx n\sqrt{\epsilon}$
    which is explained as the accumulated error of applying assertions.
\end{enumerate}
\end{theorem}

%\todo{do we need to prove the propositions/theorems}
%\begin{proof}

%\end{proof}

%{\color{red}Again, organise as a theorem here.}

==> tex/5-Efficiency.tex <==
\section{Efficiency and Robustness of Debugging}\label{sec:efficiency}
In this section, we further investigate the implementation efficiency and robustness of our projection-based assertions.
We first discuss the overhead of implementing a desired projection-based assertion accurately and propose local projection, a sound approach to simplify the assertion implementation.
We also show that projection-based assertions can be used to test and debug approximate quantum programs.

%In this section, we discuss efficient assertion designs and the decomposition of the introduced unitary transformation. We also prove the robustness of our debugging scheme. In other words, the accumulated error from the assertions is bounded when the error from each assertion is small.

%We have proved the effectiveness of projection-based assertions and shown that these assertions can be physically implemented on a quantum computer with some transformation techniques.






\subsection{Local projection: trade-off between efficiency and effectiveness}
\label{sec:efficient-implementation}
% maybe another paper
% some small projection operators
%It is very common that the projective measurement $P$ we want to implement is very hard to implement. Therefore, rather than implement $P$, we can implement a class of projective measurements $Q_1,Q_2,\cdots, Q_m$ with $Q_i\geq P$ for any $i$.
As shown in the last section, we need to manipulate the projection operators and some unitary transformations to implement an assertion.
For projections over multiple qubits, it is quite common that the qubits are highly entangled.
Asserting such entangled states requires non-trivial efforts to find the unitary transformations and we need to manipulate operators of size $2^{n}$ for an $n$-qubit system in the worst case.
%, which leads to the difficulty of implementing the unitary transformation in ICB.
However, it is possible to slightly relax the constraints in the predicates for simplified assertion implementation. % by slightly loosing the constraints in the predicates.

%To achieve this trade-off, we employ a commonly used approach in quantum information science, namely the quantum state tomography via local measurements~\cite{PhysRevLett.89.207901,PhysRevA.86.022339,PhysRevLett.118.020401}.
To achieve this trade-off, we propose local projection which  only observes part of the system.
This approach is inspired by the quantum state tomography via local measurements~\cite{PhysRevLett.89.207901,PhysRevA.86.022339,PhysRevLett.118.020401}, a common approach in quantum information science.
%To partially overcome this obstacle, we employ a commonly used approach in quantum information science, namely the quantum state tomography via local measurements  \cite{PhysRevLett.89.207901,PhysRevA.86.022339,PhysRevLett.118.020401}.
We first introduce the notion of partial trace to describe the state (operator) of a subsystem. 
Let $\overline{q}_1$ and $\overline{q}_2$ be two disjoint registers with corresponding state Hilbert space $\cH_{\overline{q}_1}$ and $\cH_{\overline{q}_2}$, respectively. 
The partial trace over $\cH_{\overline{q}_1}$ is a mapping $\tr_{\overline{q}_1}(\cdot)$ from operators on $\cH_{\overline{q}_1}\otimes\cH_{\overline{q}_2}$ to operators in $\cH_{\overline{q}_2}$ defined by:
$\tr_{\overline{q}_1}(|\phi_1\>_{\overline{q}_1}\<\psi_1|\otimes|\phi_2\>_{\overline{q}_2}\<\psi_2|) = \<\psi_1|\phi_1\>\cdot|\phi_2\>_{\overline{q}_2}\<\psi_2|$ for all $|\phi_1\>,|\psi_1\>\in\cH_{\overline{q}_1}$ and $|\phi_2\>,|\psi_2\>\in\cH_{\overline{q}_2}$ together with linearity.
The partial trace $\tr_{\overline{q}_2}(\cdot)$ over $\cH_{\overline{q}_2}$ can be defined dually. 
Then, the local projection is defined as follows:
%To illustrate this idea, we need the following definition of local projection:
%\todo{define partial trace}
\begin{definition}[Local projection]
	Given $\ass(\overline{q};P)$, a local projection $P_{\overline{q}^\prime}$ over $\overline{q}^\prime\subseteq\overline{q}$ is defined as:
	$$P_{\overline{q}^\prime} = \supp\left(\tr_{\overline{q}\backslash\overline{q}^\prime}(P)\right).$$
\end{definition}

%\begin{proposition}[Soundness of local projection]
%    For any $\rho\models P$, we have $\rho \models P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$.
%\end{proposition}
%\begin{proof}
%    Immediately from the fact $P\subseteq P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$.
%\end{proof}
\textbf{Soundness:} The $\supp()$ spans all possible states of $\overline{q}^\prime$ as well as their linear combinations, which guarantees the soundness of the local projection (we have $\rho\models P \implies \rho \models P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$, because of the fact $P\subseteq P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$).


%The $\supp()$ spans all possible states of $\overline{q}^\prime$ as well as their linear combinations, which guarantees the \textbf{soundness} of the local projection (we have $\rho\models P \implies \rho \models P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$ since $P\subseteq P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$).
%This simplification is \textbf{sound} since we have .

This simplified assertion with $P_{\overline{q}^\prime}$ will lose some checking accuracy because some states not in $P$ may be included in $P_{\overline{q}^\prime}$.
However, by taking the partial trace, we are able to focus on the subsystem of $\overline{q}^\prime$.
%Realizing that $P\subseteq P_{\overline{q}^\prime}\otimes I_{\overline{q}\backslash\overline{q}^\prime}$, 
The implementation of $\ass(\overline{q}^\prime;P_{\overline{q}^\prime})$ can partially test whether the state satisfies $P$. Moreover, the number of qubits of $\overline{q}^\prime$ is smaller and we only need to manipulate small-size operators when implementing $\ass(\overline{q}^\prime;P_{\overline{q}^\prime})$.
%and the implementation of  $\ass(\overline{q}^\prime;P_{\overline{q}^\prime})$ can be efficiently achieved.
%Therefore, 
We have the following implementation strategy which is essentially a trade-off between assertion implementation efficiency and checking effectiveness:
\begin{itemize}
	\item Find a sequence of local projection $P_{\overline{q}_1}, P_{\overline{q}_2},\cdots,P_{\overline{q}_l}$ of $\ass(\overline{q};P)$;
	\item Instead of implementing the original $\ass(\overline{q};P)$, we sequentially apply $\ass(\overline{q}_1;P_{\overline{q}_1})$, $\ass(\overline{q}_2;P_{\overline{q}_2})$, $\cdots$, $\ass(\overline{q}_2;P_{\overline{q}_l})$.
\end{itemize}
% maybe another paper
% some small projection operators
%It is very common that the projective measurement $P$ we want to implement is very hard to implement. Therefore, rather than implement $P$, we can implement a class of projective measurements $Q_1,Q_2,\cdots, Q_m$ with $Q_i\geq P$ for any $i$.

% We illustrate our idea in the following example. 
% Suppose we want to implement $P=\op{\psi}{\psi}$ where $\ket{\psi}$ is a highly entangled $n$-qubit state. 
% Now we can implement measurements $Q_{i,j}$ where $Q_{i,j}=\supp(\psi_{i,j})$ with $\psi_{i,j}$ be the reduced density matrix on qubit $i,j$ for quantum state $\ket{\psi}$.

%\iffalse
%This idea has deep connection to the quantum marginal problem. Understanding the relation between quantum marginals is considered to be one of the most fundamental problems in quantum information theory and quantum chemistry because many important physical quantities, such as energy and entropy, only depend on very
%small parts of a whole system only--these small parts are the marginal or reduced density matrices. A great deal of effort has been devoted to understanding this problem, even in the case of low dimension or a small number
%of parties. Many quantum states are uniquely determined by the support of 
%their local reduced density matrices \cite{PhysRevLett.118.020401}, which would make this idea stronger than it looks like.

%Here we can formulate the condition as follows, $\ket{\psi}$ is uniquely determined by the support of its local reduced density matrices if and only if the frustration-free Hamiltonian
%$$
%H=\sum_{i,j }I_{[n]\{i,j}\otimes Q_{i,j}
%$$
%has a unit ground state.

% Surely, other projective local measurements can also be used for approximately implementing a desire entangled projective measurement.
% \todo{pending Li's example}
% \todo{section 3.3 needs rephrase, too many new terms....}

%Let us consider a more complicated example to see how it works.
\begin{example}
Given register $\overline{q} = q_1,q_2,q_3,q_4$, we want to check if the state is the superposition of following states:
\begin{align*}
&|\psi_1\> = |+\>_{q_1}|111\>_{q_2q_3q_4},\quad |\psi_2\> = |000\>_{q_1q_2q_3}|-\>_{q_4}, \quad 
|\psi_3\> = \frac{1}{\sqrt{2}}|0\>_{q_1}\left(|00\>_{q_2q_3}+|11\>_{q_2q_3}\right)|1\>_{q_4}.
\end{align*}
To accomplish this, we may apply the assertion $\ass(\overline{q};P)$ with $P = \supp\left(\sum_{i=1}^3|\psi_i\>\<\psi_i|\right)$. However, projection $P$ is highly entangled which prevents efficient implementation. 
Observe the following local projections:
\begin{align*}
P_{q_1q_2} &= \tr_{q_3q_4}(P) = \qbit{0}{q_1}\otimes I_{q_2} + \qbit{11}{q_1q_2},\\
P_{q_2q_3} &= \tr_{q_1q_4}(P) = \qbit{00}{q_2q_3} + \qbit{11}{q_2q_3},\\
P_{q_3q_4} &= \tr_{q_1q_2}(P) = \qbit{00}{q_3q_4} + \qbit{11}{q_3q_4}.
\end{align*}
To avoid implementing $\ass(\overline{q},P)$ directly, we may apply $\ass(q_1,q_2; ~P_{q_1q_2})$, $\ass(q_2,q_3; ~P_{q_2q_3})$, and $\ass(q_3,q_4; P_{q_3q_4})$ instead. Though these assertions do not fully characterize the required property, their implementation requires only relatively low cost, i.e., each of them only acts on two qubits.
\end{example}

\subsection{Unitary transformation decomposition}
%optimization: cost 
%不同模型下的cost T count, Cnot count,...
%The additional unitary transformation is essential in \myAssertionName. 
The additional unitary transformation, which is essential in \myAssertionName, is usually decomposed into a directly supported gate set when being implemented on a quantum computer.
We focus on assertion scheme design while detailed unitary transformation decomposition is out of the scope of this paper.
Here we only briefly discuss common target gate sets for decomposition, and the metrics to evaluate a %unitary transformation 
decomposition.
%Much like any classical algorithm, a quantum algorithm needs to be implemented efficiently in order to gain maximal possible advantage from executing it.
%A unitary transformation in quantum program is usually broken down into circuits over elementary gates.
It has been proved that arbitrary unitary transformation  can be decomposed into a gate set consisting of CNOT gates and single-qubit gates~\cite{barenco1995elementary}.
CNOT gate count is a commonly used metric due to the high implementation overhead %and error rate 
of a CNOT gate under state-of-the-art technology~\cite{linke2017experimental}.

After considering quantum error correction, the set of the elementary logical gates allowed is dictated by the fault tolerance techniques that limit the efficiency of implementing an arbitrary transformation. 
Recent studies %of fault tolerance techniques 
suggest that the fault-tolerant library should consist of Clifford (single-qubit Pauli, Hadamard, Phase, CNOT gates) and T logical gates, with the understanding that the T gate requires considerably more resources than any of the Clifford gates .
It has become widely accepted that the T-gate count/depth serves as a good first-order approximation of the resource count required to physically implement a quantum circuit \cite{Aliferis:2006:QAT:2011665.2011666, Ross:2016:OAC:3179330.3179331}.



\iffalse
\subsection{Testing and debugging approximate quantum programs}\label{sec:robust}
Projection-based assertions can be used to check exact quantum programs but there are also other quantum algorithms (especially for quantum machine learning) of which the correct program states only approximately satisfy a projection.
We show that using projection-based assertions can still test and debug such approximate quantum programs.
We generalize Theorem~\ref{theorem:feasibility} by adding error parameters to represent the approximation throughout the program, and prove that we can still locate bugs or conclude about the semantics of the tested program with high confidence.


%ÈçºÎrobust µÄdebug

%Similar to the debugging scheme defined in Section~\ref{sec:debugging}, we can still use the projections $P$ and $Q$ appeared in a robust Hoare triple $\{(P,\epsilon)\}S\{(Q,\delta)\}$~\cite{zhou2019applied} to define the robust debugging scheme for approximate quantum programs while ignoring the parameter $\epsilon$ and $\delta$. 
%However, it is worthwhile to show this robust debugging scheme is still correct and efficient to detect possible errors of the program when $\epsilon$ and $\delta$ is small.
%\todo{qPCA, .......}



%We first introduce the well-known gentle measurement lemma \cite{Winter99}:
We first study a special case of the gentle measurement lemma~\cite{Winter99} with projections.
The result is slightly stronger than the original one in \cite{Winter99} under the constraint of projection.

%\textbf{Define Distance, Remove the proof to appendix}
%\begin{definition}[Trace distance of states]
%    For two states $\rho$ and $\sigma$, the trace distance $D$ between $\rho$ and $\sigma$ is defined as $$D(\rho,\sigma)=\frac{1}{2}tr|\rho-\sigma|.$$
%\end{definition}
\begin{lemma}[Gentle measurement with projections]\label{lemma:gentle}
	For projection $P$ and density operator $\rho$, if $\tr(P\rho)\ge1-\epsilon$, then	
	\begin{enumerate}
		\item $D\Big(\rho,\frac{P\rho P}{\tr(P\rho P)}\Big)\le\epsilon+\sqrt{\epsilon(1-\epsilon)}.$
		\item $F\Big(\rho,\frac{P\rho P}{\tr(P\rho P)}\Big)\ge\sqrt{1-\epsilon}.$
	\end{enumerate}
\end{lemma}

Suppose a state $\rho$ satisfies $P$ with error $\epsilon$, 
%a density operator $\rho$ is in $(P,\epsilon)$, 
then $\tr(P\rho)\ge1-\epsilon$ which ensures that, applying the projective measurement $M_P = \{M_{\bf true} = P,\ M_{\bf false} = I-P\}$, we have the outcome ``true'' with probability at least $1-\epsilon$. Moreover, if the outcome is ``true'', the post-measurement state is $\frac{P\rho P}{\tr(P\rho P)}$, which is actually close to the original state $\rho$ in the sense that their trace distance is at most $\epsilon+\sqrt{\epsilon(1-\epsilon)}$.

% Consider a program $S = S_1;S_2;\cdots;S_n$ with desired robust Hoare triples $$\{(P_0,\epsilon_0)\}S_1\{(P_1,\epsilon_1)\},\cdots, \{(P_{n-1},\epsilon_{n-1})\}S_n\{(P_n, \epsilon_n)\}$$ which are used to conclude the correctness formula 
% $\{(P_0,\epsilon_0)\}\\ S\{(P_n,\epsilon_n)\}$ of $S$. 
% The following theorem states that the debugging scheme defined in Definition \ref{debuggingscheme} is still efficient for robust debugging.

Consider a program $S = S_1;S_2;\cdots;S_n$ with $n$ inserted assertions $\ass(\overline{q}_m,P_m)$ after each segments $S_i$ for $1\le m\le n$. Unlike the exact algorithms, here each program segment $S_m$ is considered to be correct if its input satisfies $P_{m-1}$, then its output approximately satisfies $P_m$ with error parameter $\epsilon_m$.
The following theorem states that the debugging scheme defined in Definition \ref{debuggingscheme} is still effective for debugging approximate quantum programs.

\begin{theorem}[Feasibility of robust debugging]\label{theorem:robust}

Assume that all $\epsilon_i$ are small. %, say $\epsilon_i\le\epsilon$. 
Execute $S^\prime$ for $k$ times ($k \gg n^2$) with input $\rho$, and we count $k_m$ for the occurrence of error message for assertion $\ass(\overline{q}_m, P_m)$. 
\begin{enumerate}
    \item The 95\% confidence interval of real $\epsilon_m$ is $[w_m^-,w_m^+]$. Thus, with confidence 95\%, if $\epsilon_m<w_m^-$, we conclude $S_m$ is incorrect; and if $\epsilon_m>w_m^+$, we conclude $S_m$ is correct. Here, $w_m^-, w_m^+$ and $w_m^c$ are $B\left(\alpha, k_m+1, k - \sum_{i=1}^{m}k_i\right)$ with $\alpha = 0.025,0.975$ and $0.5$ respectively, where $B(P,A,B)$ is the $P$th quantile from a beta distribution with shape parameters $A$ and $B$.
    %\item If $\frac{k_m}{k-\sum_{i=0}^{m-1}k_i}$ is significantly larger than $\epsilon_m$, we conclude that $S_m$ is not valid for $\{(P_{m-1},\epsilon_{m-1})\}S_m\{(P_m,\epsilon_m)\}$ with high confidence.
    
    \item If no segment appears to be incorrect, i.e., all $\epsilon_m\ge w_m^-$, then after executing the original program $S$ with input $\rho$, the output state $\sigma$ approximately satisfies $P_n$ with error parameter $\delta$, i.e., $\sigma\models_\delta P_n$, where $\delta = \sum_{m=1}^n\sqrt{w_m^c} + \sqrt{\sum_{m=1}^n(\sqrt{w_m^+}-\sqrt{w_m^c})^2}$. 
    
    
    % \item If all $\frac{k_m}{k-\sum_{i=0}^{m-1}k_i}$ are close to or smaller than $\epsilon_m$ for all $m\ge1$, we can conclude that %$\{(P_0,\epsilon_0)\}S\{(P_n,\epsilon_n+\delta)\}$ 
    % $\{(P_0,0)\}S\{(P_n,\delta)\}$ 
    % is valid with high probability, where 
    % $\delta = \sum_{i=1}^n\big(\epsilon_i+\sqrt{\epsilon_i(1-\epsilon_i)}\big) \approx \sum_{i=1}^n\sqrt{\epsilon_i}$
    % %$\delta = n(\epsilon+\sqrt{\epsilon(1-\epsilon)})\approx n\sqrt{\epsilon}$
    % which is explained as the accumulated error of applying assertions.
\end{enumerate}
\end{theorem}

\begin{proof}
Postponed to Appendix~\ref{proof:robust}
\end{proof}


With this theorem, we can test and debug approximate quantum programs by counting the number of occurrence of the error messages from different assertions.
If the observed assertion checking failure frequency is significantly higher or lower than the expected error parameter of a program segment, we can conclude that this program segment is correct or incorrect with high confidence.
If all program segments appear to be correct, we can conclude that the final output of the original program is approximately satisfies that last predicate with a bounded error parameter.

\fi
%\todo{}

%\todo{do we need to prove the propositions/theorems}
%\begin{proof}

%\end{proof}

%{\color{red}Again, organise as a theorem here.}

==> tex/5-OverallImprovement.tex <==
\section{Overall Comparison}\label{sec:overall}
We evaluate \myAssertionName~in the Section~\ref{sec:overall} and~\ref{sec:casestudy}.
In this section, we focus on an overall comparison among \myAssertionName~and two other quantum program assertions in terms of assertion coverage (i.e., the expressive power of the predicates, the assertion locations in a program) and debugging overhead (i.e., the number of measurements, executions, and auxiliary qubits).

\textbf{Baseline}
We use the statistical assertions~(Stat)~\cite{huang2019statistical} and the QEC-inspired assertions~(QECA)~\cite{zhou2019quantum} as the baseline assertion schemes. 
To the best of our knowledge, they are the only published quantum program assertions till now.
Stat employs classical statistical test on the measurement results to check if a state satisfies a predicate. % specified in the assertion.
QECA introduces auxiliary qubits to indirectly measure the tested state.

%They are compared with the projection-based assertion~(Proj) proposed in this paper.

\iffalse
In this section, we evaluate the assertions against existing quantum program assertion schemes.
We start from an overall analysis to compare the proposed assertion scheme and other assertion schemes 


Then, we demonstrate the usage of the proposed assertion and debugging scheme on two realistic sophisticated quantum algorithms, Shor's algorithm~\cite{shor1999polynomial} and HHL algorithm~\cite{harrow2009quantum}.
For Shor's algorithm, we will show how the assertions are injected in a quantum program and how they are implemented.
We also compare the implementation cost of \myAssertionName~and QECA when applying on Shor's algorithm to show the efficiency of \myAssertionName.
For HHL algorithm, since it is more complicated and the derived assertions are not supported in other existing assertion schemes, we focus on the numerical results to illustrate how the projection implementation techniques introduce in Section~\ref{sec:debugging} are applied.




Before getting into concrete examples, we first compare the proposed assertion scheme \myAssertionName~with the baseline schemes in terms of assertion coverage and debugging overhead in general.
\fi


\subsection{Coverage analysis}
\textbf{Assertion predicates} \myAssertionName~employs projections which are able to represent a wide variety of predicates in the derived assertions.
However, both Stat and QECA only support three types of assertions: classical assertion, superposition assertion, and entanglement assertion.
All these three types of assertions can be considered as 1-dimensional special cases in \myAssertionName.
The corresponding projections are
\begin{align*}
    &P=\ket{t}\bra{t}, \text{t ranges over all n-bit strings} \\
    &\quad\text{for classical assertion~(suppose n qubits are asserted)}  \\
    &P=\ket{+\!+\!+\dots}\bra{+\!+\!+\dots} \text{ for superposition assertion} \\
    &P=(\ket{00\dots0}+\ket{11\dots1})(\bra{00\dots0}+\bra{11\dots1})  \\ 
    & \quad \text{for entanglement assertion}
\end{align*}
%$P=\ket{x_1 x_2 \dots x_n}\bra{x_1 x_2 \dots x_n}, x_i\in\{0,1\}, 1 \leq i \leq n$ for classical assertion, $P=\ket{+++\dots}\bra{+++\dots}$ for superposition assertion, and $P=(\ket{00\dots0}+\ket{11\dots1})(\bra{00\dots0}+\bra{11\dots1})$ for entanglement assertion.
Thus, all the three types of assertions are covered in \myAssertionName. 
The expressive power of the assertions in \myAssertionName, which can support many more complicated cases as introduced in Section~\ref{sec:debugging}, is much more than that of the baseline schemes.

%For the assertion location, \myAssertionName~can inject assertions at arbitrary place in a program with the help of the proof system proposed in aQHL~\cite{zhou2019applied}.
\textbf{Assertion locations} 
Thanks to the expressive power of the predicates in \myAssertionName, there is no limitation on the assertion locations for \myAssertionName.
But the baseline schemes can only inject assertions in those places with states that can be checked with the very limited types of assertions.
If the baseline schemes insert assertions at locations with other types of states, their assertions will always return negative results since the predicates in their assertions are not correct.
Therefore, the number of potential assertion injection locations of \myAssertionName~is much larger than that of the baseline schemes. 

\begin{table}[h]
  \centering
  \vspace{-5pt}
  \caption{Asymptotic overhead comparison for \myAssertionName, Stat~\cite{huang2019statistical}, and QECA~\cite{zhou2019quantum}, $m$ assertions, $n$ qubits, and $N \gg 2^{n}$ }%Suppose there are $n$ qubits, $m$ assertions (supported by all three assertion schemes), and the number of executions for one statistical test is $N$ (usually very large).}
   \vspace{-10pt}
    \begin{tabular}{|c||c|c|c|}
    \hline
     \# of     & \myAssertionName  & Stat  & QECA  \\
    \hline
    \hline
    Measure & $O(nm)$ & $O(nmN)$ & N/A \\
    \hline
    Execution & $O(1)$  & $mN$    & N/A \\
    \hline
    Aux. Qbit & $0$ or $1$     & $0$     & $ \geq 1$ \\
    \hline
    \end{tabular}%
    \vspace{-10pt}
  \label{tab:asym_overhead_analysis}%
\end{table}%

\subsection{Debugging overhead analysis}
To analyze the debugging overhead of the three assertion schemes, we assume that all the assertions are within the three types of assertions supported in all assertion schemes in order to perform a fair overhead comparison.
Suppose there are $n$ qubits in the program with $m$ assertions injected. 
For Stat, we suppose that the number of executions for one statistical test is $N$.
Usually we have $N \gg 2^{n}$ to ensure an accurate estimation for the $2^{n}$ amplitudes in the state vector.





Table~\ref{tab:asym_overhead_analysis} shows the asymptotic overhead comparison for \myAssertionName, Stat~\cite{huang2019statistical}, and QECA~\cite{zhou2019quantum}.
In particular, we compare the number of measurement operations (here one measurement operation means measuring one qubit), executions, and auxiliary qubits.
Among them, Stat is the most time consuming one which requires $mN$ executions and $O(mnN)$ measurements because each time only one out of the $m$ assertions is checked (with $O(n)$ measurements) and for each assertion Stat needs to run $N$ repeated executions.
But for \myAssertionName, in each execution all $m$ assertions (with $O(n)$ measurements for each assertion) can be checked and only $O(1)$ executions will reveal unsatisfied assertions with a high probability.
The total number of measurements would be $O(nm)$.
QECA does not provide a complete implementation of debugging with multiple assertions.
%Thus the number of executions for them is $O(1)$ and the number of measurements is $O(mn)$.
For the number of auxiliary qubits, Stat does not require any auxiliary qubits while QECA requires at least one additional qubit.
For \myAssertionName, at most one auxiliary qubit is enough when $\rank P>2^{n-1}$.
%\todo{}

In summary, \myAssertionName~significantly outperforms both Stat and QECA with much stronger expressive power and flexible assertion location.
Also, \myAssertionName~is much more efficient than the time-consuming Stat.
We do not compare with QECA comprehensively but 
%Compared with QECA, \myAssertionName~does not show much advancement in the asymptotic overhead analysis.
later in the case study of Shor's algorithm, we will show that the implementation of \myAssertionName~has much lower overhead than that of QECA.

==> tex/6-CaseStudy.tex <==
\section{Case Studies: Runtime Assertions for Realistic Quantum Algorithms}\label{sec:casestudy}

%In the last section, we have already shown the 
In this section, we perform case studies by appling~\myAssertionName~on two famous sophisticated quantum algorithms, the Shor's algorithm~\cite{shor1999polynomial} and the HHL algorithm~\cite{harrow2009quantum}.
We will demonstrate how to derive assertions with \myAssertionName~and how the assertions work in these realistic programs.

For Shor's algorithm, we focus the circuit implementation of the assertions injected in a concrete example of the quantum order finding subroutine. 
%Since 
The derived assertions are simple and can be supported by the baselines, which allows us to compare the resource consumption between \myAssertionName~and the baseline and show that \myAssertionName~could generate low overhead runtime assertions.

For HHL algorithm, instead of just asserting a concrete circuit implementation, we will show that \myAssertionName~could derive non-trivial assertions that cannot be supported by the baselines.
In these non-trivial assertions, we will illustrate how the proposed techniques, i.e., combining assertions, auxiliary qubits, local projection, can be applied in implementing the projections.
Numerical simulation confirms that \myAssertionName-derived assertions can work correctly.



\subsection{Shor's algorithm}\label{sec:shor}
Shor's algorithm was proposed to factor a large integer~\cite{shor1999polynomial}. Given an integer $N$, Shor's algorithm can find its non-trivial factors within $O(poly(log(N)))$ time.
In this paper, we focus on its quantum order finding subroutine % in Shor's algorithm 
and omit the classical part which is assumed to be correctly implemented.
%We assume that the classical subroutine is correct. 
%a
%The classical subroutine is assumed to be correctly implemented.

%We also assume that the classical subroutine is implemented correctly since the testing and verification of classical programs is out of the scope of this paper. % it could be checked with mature testing and verification techniques in classical computing..

\subsubsection{Shor's algorithm program}
Figure~\ref{fig:shor} shows the program of the quantum subroutine in Shor's algorithm with the injected assertions in the quantum {\bf while}-language.
Briefly, it leverages Quantum Fourier Transform~(QFT) to find the period of the function $f(x) = a^{x}~{\rm mod}~N$ where $a$ is a random number selected by a preceding classical subroutine.
The transformation $U_f$, the measurement $M$, and the result set $R$  are defined as follows:

\begin{align*}
U_f &:\ \ket{x}_{p}\ket{0}_{q} \mapsto \ket{x}_{p}\ket{a^{x}~{\rm mod}~N}_{q}\\
M&=\Big\{M_{0} = \sum_{r\in R}\ket{r}\bra{r}, M_{1}=I-M_{0}\Big\}\\
R&=\{r~|~{\rm gcd}(a^{\frac{r}{2}} + 1,N) ~{\rm or~gcd}(a^{\frac{r}{2}} - 1,N) \\
& \qquad \text{is a nontrivial factor of N}  \}
\end{align*}
For the measurement, the set $R$ consists of the expected values that can be accepted by the follow-up classical subroutine.
For a comprehensive introduction, please refer to~\cite{nielsen2010quantum}.

\begin{figure}[t]
\centering
\begin{align*}
&p := |0\>^{\otimes n};\\
&{\rm\bf while\ }M[p] = 1 {\ \rm\bf do\ } \\
&\qquad p := |0\>^{\otimes n};\ q := |0\>^{\otimes n};\\
&\qquad \ass(p,q; A_{0}); \\
&\qquad p := H^{\otimes n}[p]; \\
&\qquad \ass(p,q; A_{1}); \\
%&q := X^{\otimes n}[q]; \\
&\qquad p,q := U_f[p,q];   \\
&\qquad \ass(p,q; A_{2}); \\
&\qquad p := {\rm QFT}^{-1}[p];  \\
&\qquad \ass(p,q; A_{3}); \\
&{\ \rm\bf od\ }
\end{align*}
\vspace{-20pt}
\caption{Shor's algorithm program with assertions}\label{fig:shor}
\vspace{-10pt}
\end{figure}


\begin{figure*}[t]
\centering
%\vspace{-10pt}
\includegraphics[width=1.0\columnwidth]{fig/shor-crop.pdf}
\vspace{-10pt}
\captionsetup{justification=centering}
\caption{Assertion-injected circuit implementation for Shor's algorithm with $N=15$ and $a=11$}
\vspace{-10pt}
\label{fig:shor_circuit}
\end{figure*}

\subsubsection{Assertions for a concrete example}
The circuit implementation we select for the subroutine is for factoring $N=15$ with the random number $a=11$~\cite{vandersypen2001experimental}.
This will not lose the generality since the overall circuit structures for other configurations are similar.
We apply \myAssertionName~on this circuit and derive four assertions, $A_{0}$, $A_{1}$, $A_{2}$, and $A_{3}$, as shown in Figure~\ref{fig:shor}.
The proof outline is in Appendix~\ref{appendix:shor}.



Figure~\ref{fig:shor_circuit} shows the final assertion-injected circuit with 5 qubits.
The circuit blocks labeled with $\bf assert$ are for the four assertions with four projections defined as follows:
\begin{align*}
A_{0} &= \qbit{00000}{0,1,2,3,4};\\
A_{1} &= \ket{+\!+\!+}_{0,1,2}\bra{+\!+\!+} \otimes \qbit{00}{3,4}; \\
A_{2} &= \ket{+\!\,+}_{0,1}\bra{+\!\,+} \otimes (\ket{000}+\ket{111})_{2,3,4}(\bra{000}+\bra{111}); \\
A_{3} &= (\ket{000}+\ket{001})_{0,1,2}(\bra{000}+\bra{001}) \otimes (\ket{00}+\ket{11})_{3,4}(\bra{00}+\bra{11}).
\end{align*}
We detail the implementation of the assertion circuit blocks on the upper half of Figure~\ref{fig:shor_circuit}.
For each assertion, we list its projection, the additional unitary transformations, with the complete implementation circuit diagram.
For $A_{1}$, $A_{2}$, and $A_{3}$, since the qubits not fully entangled, we only assert part of the qubits without affecting the results.
The unitary transformations are decomposed into the combinations of CNOT gates and single-qubit gates by hand.

%As introduced in Section~\ref{sec:debugging}, we can debug the shor's algorithm program 

%\todo{Gushu will finish this}


\iffalse

\subsection{Shor's Algorithm}
%\todo{simple, uncorrelated loop body}
%Shor's algorithm contains both classical subroutines and one quantum subroutine.
We focus on assertion injection for the quantum order finding subroutine in Shor's algorithm as introduced in Section~\ref{sec:assertion}.
In particular, the circuit implementation we selected for the subroutine is for factoring $N=15$ with the random number $a=11$~\cite{vandersypen2001experimental} with loss of generality since circuits for other configurations are similar.
Totally four assertions are derived and injected across the circuit.
The classical part in Shor's algorithm is assumed be correct since it could be checked with mature testing and verification techniques in classical computing.
\fi



%On the bottom is an overview of the constructed circuit.




\subsubsection{Assertion comparison}
Similar to Section~\ref{sec:overall}, we first compare the coverage of assertions derived for this realistic algorithm, and then detail the implementation cost in terms of the number of additional gates, measurements, and auxiliary qubits.

\textbf{Assertion Support}
All four assertions are supported in Stat and \myAssertionName.
For QECA, $A_0$, $A_{1}$, and $A_3$ are covered but $A_2$ is not yet supported even if it is an entanglement state. Because the assertion from QECA for the two-qubit entanglement state cannot be directly extended to cases with more qubits.

\textbf{Implementation Cost}
We compare the circuit cost when implementing the assertions between \myAssertionName~and QECA. 
Stat is not included because it only requires some additional measurements and we have already shown the inefficiency of Stat with respect to the numbers of executions in Section~\ref{sec:overall}.

\begin{table}[b]
  \centering
  \vspace{-10pt}
  \caption{Detailed assertion implementation cost comparison between \myAssertionName~and QECA~\cite{zhou2019quantum} for assertion $A_0$, $A_{1}$, and $A_3$}% in the Shor's algorithm example}%. Note that assertion $A_2$ is not yet supported in QECA.}
  \vspace{-10pt}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
          & \multicolumn{2}{c|}{$A_{0}$} & \multicolumn{2}{c|}{$A_{1}$} & \multicolumn{2}{c|}{$A_{3}$} \\
    \hline
     \# of     & \myAssertionName & QECA  & \myAssertionName  & QECA  & \myAssertionName  & QECA \\
   \hline
    H     & 0     & 0     & 6     & 6     & 2     & 2 \\
    \hline
     \textbf{CNOT } & \textbf{0}     & \textbf{5}     & \textbf{0}     & \textbf{6}     & \textbf{0}    & \textbf{4}\\
    \hline
    Measure & 5     & 5     & 3     & 3     & 3     & 3 \\
    \hline
  \textbf{ Aux. Qbit}  & \textbf{0}     & \textbf{1}     & \textbf{0}     & \textbf{1}   & \textbf{0}     & \textbf{1} \\
    \hline
    \end{tabular}%
     %\vspace{-5pt}
  \label{tab:detailed_gate_cost}%
\end{table}%

Table~\ref{tab:detailed_gate_cost} shows the implementation cost of the three assertions supported by both \myAssertionName~and QECA.
In particular, we compare the number of H gates, CNOT gates, measurements, and auxiliary qubits.
It can be observed that \myAssertionName~use no CNOT gates and auxiliary qubits for the three considered assertions, while QECA always needs to use additional CNOT gates and auxiliary qubits.
This reason is that QECA always measure auxiliary qubits to indirectly probe the qubit information. So that additional CNOT gates are always required to couple the auxiliary qubits with existing qubits.
This design significantly increases the implementation cost when comparing with \myAssertionName.

%\subsubsection{Comparison with other assertions}
%We compare the projection-based assertion proposed in this paper~(Proj), with statistical assertions~(Stat) and QECC-inspired assertions~(QECA).

%\textbf{Assertion Type Coverage}








%

% 
To summarize, we demonstrate the complete assertion-injected circuit for a quantum program of Shor's algorithm and the implementation details of the assertions.
We compare the implementation cost between \myAssertionName~and QECA to show that \myAssertionName~has lower cost even for the limited assertions that are supported by both assertion schemes.

\subsubsection{Bug Injection Experiments and Results}


\todo{}



\subsection{HHL algorithm}
% introduce HHL, proof outline, while loop invariant decomposition
%In the first example of asserting Shor's algorithm program, we have demonstrated how to use \myAssertionName~with a concrete example. 
%We focused on the circuit implementation and the comparison against the baseline since the derived assertions have simple form.
In the first example of Shor's algorithm, we focus the assertion implementation on a concrete circuit example and compare against other assertions due to the simplicity of the derived assertions.
In the next HHL algorithm example, we will have non-trivial assertions that are not supported in the baselines and demonstrate how to implement the projection with the techniques introduced in Section~\ref{sec:debugging} and~\ref{sec:efficient-implementation}.

%In this section we will show how to use the assertions to perform runtime tests on the so-called HHL algorithm.
The HHL algorithm was proposed for solving linear systems of equations~\cite{harrow2009quantum}. 
Given a matrix $A$ and a vector $\vec{b}$, the algorithm produces a quantum state $|x\>$ which is corresponding to the solution $\vec{x}$ such that $A\vec{x}=\vec{b}$. 
It is well-known that the algorithm offers up to an exponential speedup over the fastest classical algorithm if $A$ is sparse and has a low condition number $\kappa$.



\begin{figure}[t]
	\centering
	\begin{align*}
	&p := |0\>^{\otimes n};\ q := |0\>^{\otimes m};\ r := |0\>;\\
%	&\ass(p,q,r; R); \\
	&{\rm\bf while\ }M[r] = 1 {\ \rm\bf do\ } \\
	&\qquad \ass(p,r; P); \\
%	&\qquad \\
	&\qquad q := |0\>^{\otimes m};\ q := U_b[q];\ p := H^{\otimes n}[p]; \\
	&\qquad p,q := U_f[p,q]; \ p := {\rm QFT}^{-1}[p]; \\
%	&\qquad   \\
	&\qquad \ass(p; S);  \\
	&\qquad p,r := U_c[p,r]; \ p := {\rm QFT}[p];  \\
	%&\qquad   \\
	&\qquad p,q := U_f^{\dag}[p,q]; \ p := H^{\otimes n}[p];  \\
	%&\qquad  \\
	&\qquad \ass(p,q,r; R); \\
	&{\rm\bf od\ } \\
	&\ass(q; Q);
	\end{align*}
	\vspace{-20pt}
	\caption{HHL algorithm program with assertions}\label{fig:hhl}
	\vspace{-10pt}
\end{figure}


\begin{figure*}[t]
\centering
%\vspace{-10pt}
\includegraphics[width=1.0\columnwidth]{fig/hhl-crop.pdf}
\vspace{-7pt}
\captionsetup{justification=centering}
\caption{Numerical simulation results for the states around the assertions in HHL algorithm}
\vspace{-10pt}
\label{fig:hhl_result}
\end{figure*}


\subsubsection{HHL program}

The HHL algorithm has been formulated to the quantum {\bf while}-language and formally statically verified in the sense of both partial and total correctness in~\cite{zhou2019applied}. 
We adopt the assumptions and symbols there.
Briefly speaking, $A$ is a Hermitian and full-rank matrix with dimension $N = 2^m$, which has the diagonal decomposition $A = \sum_{j=1}^N\lambda_j|u_j\>\<u_j|$ with corresponding eigenvalues $\lambda_j$ and eigenvectors  $|u_j\>$.
We assume for all $j$, $\delta_j = \frac{\lambda_jt_0}{2\pi}\in\mathbb{N}^+$ and set $T = 2^n = \lceil\max_j\delta_j\rceil$, where $t_0$ is a time parameter to perform unitary transformation $U_f$. Moreover, the input vector $\vec{b}$ is presumed to be unit and corresponding to state $|b\>$ with the linear combination $|b\> = \sum_{j=1}^N\beta_j|u_j\>$. It is straightforward to find the solution state $|x\> = c\sum_{j=1}^N\frac{\beta_j}{\lambda_j}|u_j\>$ where $c$ is for normalization.
%with unimportant scale factor $c$ used to normalize $|x\>$.

The HHL program has three registers $p,q,r$ which are $n,m,1$-qubit systems and used as the control system, state system and indicator of while loop, respectively. For details of unitary transformations $U_b,U_f$ and ${\rm QFT}$ and measurement $M$, please refer to Appendix~\ref{appendix:hhl} or \cite{zhou2019applied,harrow2009quantum}. 





\subsubsection{Debugging scheme for HHL program}
According to the proof outline for HHL program in \cite{zhou2019applied} (also in Appendix~\ref{appendix:hhl}), %\todo{put in appendix}
we introduce the debugging scheme shown in Figure \ref{fig:hhl}. % based on Definition \ref{debuggingscheme}. 
The projections $R,P,Q,S$ are defined as follows:
\begin{align*}
&P = \qbit{0}{p} \otimes \qbit{0}{r};\ Q = \qbit{x}{q}; \\
&R = \qbit{0}{p} \otimes (\qbit{x}{q}\otimes\qbit{1}{r} + I_q\otimes \qbit{0}{r}); \\
&S = \supp\left(\sum_{j=1}^N\qbit{\delta_j}{p}\right).
\end{align*}
Projection $R$ is the same as in \cite{zhou2019applied} while $P$ is focused on register $p,r$ and $Q$ is focused on the output register $q$. These projections can be implemented using the techniques introduced in Section~\ref{sec:debugging}; more precisely:
\begin{enumerate}
	\item Implementation of $\ass(p,r; P)$:
		
		measure register $p$ and $r$ directly to see if the outcomes are all ``0'';
		
	\item Implementation of $\ass(q; Q)$:
		
		apply $U_x$ on $q$;
		
		measure register $q$ and check if the outcome is ``0'';
		
		apply $U_x^\dag$ on $q$;
		
	\item Implementation of $\ass(p,q,r; R)$:
		
		measure register $p$ directly to see if the outcome is ``0'';
		
		introduce an auxiliary qubit $a$, initialize it to $|0\>$;
		
		apply $U_x$ on $q$ and $U_R$ on $r,q,a$;
		
		measure register $a$ and check if the outcome is ``0'';
		
		apply $U_R^\dag$ on $r,q,a$ and $U_x^\dag$ on $q$;
\end{enumerate}
where $U_x$ is defined by $U_x|x\> = |0\>$
and $U_R$ is defined by
$$U_R\qbit{1}{r}\otimes\qbit{i}{q}\otimes\qbit{k}{a} = \qbit{1}{r}\otimes\qbit{i}{q}\otimes\qbit{k\oplus1}{a}$$
for $i\ge1$ and $k=1,2$
and unchanged otherwise. In fact, when implementing $\ass(p,q,r; R)$, $p$ can also be used as the auxiliary qubit $a$ since $p$ is in $|0\>$.
%note that $p$ is in $|0\>$ and therefore, $p$ can also be used as the auxiliary qubit $a$.

We need to pay more attention to $\ass(p; S)$. The original predicate here is
$S^\prime = \sum_{j,j^\prime=1}^N \beta_j\overline{\beta}_{j^\prime}|\delta_j\>_p\<\delta_{j^\prime}|\otimes |u_j\>_q\<u_{j^\prime}|\otimes \qbit{0}{r},$
which is a highly entangled projection over register $p$ and $q$. 
As discussed in Section \ref{sec:efficient-implementation}, in order to avoid the hardness of implementing $S^\prime$, we introduce $S = \supp(\tr_{q,r}(S^\prime))$ which  is actually  the reduced projection of $S^\prime$ over $p$. Though $\ass(p; S)$ is strictly weaker than original $\ass(p,q,r; S^\prime)$, it can be efficiently implemented and partially test the state.

%\section{Evaluation}\label{sec:evaluation}



%\textbf{Metrics}
%We will first assess the \textbf{Assertion Coverage}
%For those assertions that can be supported by all the three assertion schemes, 









\subsubsection{Numerical simulation results}
For illustration, we choose $m=n=2$ as an example.
Then the matrix $A$ is $4\times4$ matrix and $b$ is $4\times 1$ vector. 
We first randomly generate four orthonormal vectors for $\ket{u_{j}}$ and then select $\delta_{j}$ to be either 1 or 3.
Such configuration will demonstrate the applicability of all four derived assertions.
Finally, $A$ and $b$ are generated as follows. 
% \todo{how to generate for Assertion S}
% implementation, circuit, result distribution
$$A = 
\begin{bmatrix}
1.951 & -0.863 & 0.332 & -0.377 \\
    -0.863 & 2.239 & -0.011 & -0.444 \\
    0.332 & -0.011 & 1.301 & -0.634 \\
    -0.377 & -0.444 & -0.634 & 2.509 
\end{bmatrix}
, b =
\begin{bmatrix}
    -0.486 \\
    -0.345 \\
    -0.494 \\
    -0.633 
\end{bmatrix}
$$

\textbf{Assertion Support}
We have four assertions, labeled $P$, $Q$, $R$, and $S$, for the HHL program. 
Only $P$ is for a classical state and supported by the baselines and \myAssertionName.
$Q$, $R$, and $S$ are more complex and not supported in the baselines.


Figure~\ref{fig:hhl_result} shows the amplitude distribution of the states during the execution of the four assertions and each block corresponds to one assertion.
Since our experiments are performed in simulation, we can directly obtain the state vector $\ket{\psi}$. % in the simulator. 
The X-axis represents that basis states of which the amplitudes are not zero.
The Y-axis is the probability of the measurement outcome,
This probability 
%which 
can be calculated by $\left\Vert\bra{\psi}\ket{x}\right\Vert^{2}$, where $\ket{x}$ is the corresponding basis state.


%Then We obtain the measurement results distribution of some states around the assertion based on the state vector in the simulator.

\textbf{Assertion P} is at the beginning of the loop body $D$. 
%in Figure we demonstrate the Assertion P is at the beginning of the loop body $D$. 
The predicate is $P=\ket{000}_{r,p}\bra{000}$, which has a simple classical form but requires non-trivial efforts to find that the quantum register $p$ is always in state $\ket{00}$ at the beginning of the loop body. 
%The derivation process is in the Appendix~\ref{appendix:hhl}.
%This fact could be found with \myAssertionName~but it is hard to derive such assertions in Stat and QECA. 
%The results in 
Figure~\ref{fig:hhl_result} shows that when the program enter the loop $D$ at the first and second time, the assertion is satisfied and the quantum registers $r$ and $q$ are 0.

\textbf{Assertion Q} is at the end of the program. 
Figure~\ref{fig:hhl_result} shows that there are non-zero amplitudes at 4 possible measurement outcomes at the assertion location. But after the applied unitary transformation, the only possible outcome is $10000$. 
Such an assertion is hard for Stat and QECA to describe but it is easy to define this assertion using projection in \myAssertionName.

\textbf{Assertion R} is at the end of the loop body $D$.
Figure~\ref{fig:hhl_result} confirms that the basis states with non-zero amplitudes are in the subspace defined by the projection in assertion R.
Its projection implementation involves the techniques of combining assertions and using auxiliary qubits.
Assertions with such complex predicates cannot be defined in Stat and QECA while \myAssertionName~can decompose and implement it.

\textbf{Assertion S} is in the middle of the loop body $D$.
At this place the state is highly entangled as mentioned above and directly implementing this projection will be expensive.
We employ the local projection technique in Section~\ref{sec:efficient-implementation}. % and 
Since $\delta_{j}$s are selected to be either 1 or 3, the projection $S$ becomes $\qbit{01}{p}+\qbit{11}{p}$.
This simple form of local projection that can be easily implemented.
Figure~\ref{fig:hhl_result} confirms that the tested highly entangled state is not affected in this local projective measurement.

To summarize, we derive four assertions for the program of HHL algorithm with \myAssertionName.
Among them, only $P$ can be defined in Stat and QECA but it is hard to realize the predicate in this assertion without the help of quantum logic.
The rest three assertions, which cannot be defined in Stat or QECA, demonstrate that \myAssertionName~%and the proposed techniques 
can help assert and debug realistic quantum algorithms on a quantum computer.



%\todo{Gushu will finish this after doing the experiment for assertion S}







==> tex/7-Discussion.tex <==
\section{Discussion}\label{sec:discussion}

Program debugging has been an active research topic for a long time because it reflects the practical application requirements for reliable software.
Compared with its counterpart in classical computing, quantum program debugging is still at a very early stage.
Basic debugging approaches, such as assertions~\cite{clarke2006historical}, static code analysis~\cite{bessey2010few}, and design by contract~\cite{meyer1992applying}, which have been invented for classical program debugging in the last few decades, are not yet available or well-developed for quantum programs.
This paper made efforts towards practical quantum program debugging through studying how to design and implement effective and efficient quantum program assertions. % to help with quantum program debugging.
Specifically, we select projections as predicates in our assertions.
Several techniques are proposed to implement the projection under machine constraints.
To the best of our knowledge, this is the first runtime assertion scheme for quantum program debugging with such flexible assertions and low testing overhead.
The proposed assertion technique would benefit future quantum program development, testing, and verification.

Although we have demonstrated the feasibility and advantages of the proposed assertion scheme, there are several future research directions that can be explored as with any initial research.

\textbf{Projection Implementation Optimization}
We have sh-own that our assertion-based debugging scheme can be implemented with several techniques in Section~\ref{sec:debugging} and demonstrated concrete examples in Section~\ref{sec:casestudy}.
However, further optimization of the projection implementation is not yet well studied.
One assertion can be split into several sub-assertions but different sub-assertion selections would have different implementation overhead.
We showed that one auxiliary qubit is enough but employing more auxiliary qubits may yield fewer sub-assertions.
For the circuit implementation of an assertion, the decomposition of the assertion-introduced unitary transformations can be optimized for several possible objectives, e.g., gate count, circuit depth.
A systematic approach to generate optimized assertion implementations is thus important for more efficient assertion-based quantum program debugging in the future.

\textbf{More Efficient Checking}
Assertions derived from \myAssertionNameSpace for a complicated highly entangled state may require significant effort for its precise implementation.
However, the goal of assertions is to check if a tested state satisfies the predicates rather than to prove the correctness of a program.
It is possible to trade-in checking accuracy for simplified assertion implementation by relaxing the constraints in the predicates.
Local projection can be a solution to approximate a complex projective measurement as we discussed in Section~\ref{sec:efficient-implementation} and demonstrated in one of the assertions for the HHL algorithm in Section~\ref{sec:casestudy}.
However, the degree of predicate relaxation and its effect on the robustness of the assertions %how much we should relax in the predicates and how it will affect the robustness of the assertions 
in realistic erroneous program debugging need to be studied.
Other possible directions, like non-demolition measurement~\cite{braginsky1980quantum}, are also worth exploring.
%\todo{read [35]}


%\todo{add more about local hamiltonian}
%, e.g., $T$ gate count, $CNOT$ gate count, overall
%cooperate with logic system
%can be easily integrated into existing quantum programming languages


%Debugging on classical computer

%Assertion can detect error but cannot guarantee the correctness.

%implementation cost, number of projections, number of auxiliary qubits

==> tex/8-RelatedWork.tex <==
\section{Related Work}\label{sec:relatedwork}

This paper explores runtime assertion schemes for testing and debugging a quantum program on a quantum computer.
In particular, the efficiency and effectiveness of our assertions come from the application of projection operators.
Therefore, in this section, We first introduce other existing runtime quantum program testing schemes, which are the closest related work, and then briefly discuss other quantum programming techniques involving projection operators.
%and then briefly cover the application of projections in other quantum program 

%This paper explores logic-assisted assertion design schemes for debugging on a quantum computer.
%In this section, we briefly discuss related work.

%\subsection{Assertions for Quantum Programming}
%\todo{this section may move}

\subsection{Runtime quantum program testing schemes}
Recently, two types of assertions have been proposed for debugging on quantum computers.
Huang and Martonosi proposed quantum program assertions based on statistical tests on classical observations~\cite{huang2019statistical}.
For each assertion, the program executes from the beginning to the place of the injected assertion followed by measurements. This process is repeated many times to extract the statistical information about the state. 
The advantage of this work is that, for the first time, assertion is used to reveal bugs in realistic quantum programs and help discover several bug patterns.
But in this debugging scheme, each time only one assertion can be tested due to the destructive measurements. 
Therefore, the statistical assertion scheme is very time consuming. 
%The scheme described in this paper 
\myAssertionNameSpace circumvents this issue by choosing to use projective assertions.

Zhou and Byrd further improved the assertion scheme by proposing dynamic assertion circuits inspired by quantum error correction~\cite{zhou2019quantum}.
They introduce ancilla qubits and indirectly collect the information of the qubits of interest.
The success rate can also be improved since some unexpected states can be detected and corrected in the noisy scenarios.
However, their approach always relies on ancilla qubits, which will increase the implementation overhead as discussed in Section~\ref{sec:shor}.% only provide assertion circuits ir% \todo{}%assertion \todo{small size}

Moreover, both of these assertion schemes can only inspect very few types of states that can be considered as some 1-dimensional special cases of our proposed projection based assertions, leading to limited applicability. 
In summary, our assertion and debugging schemes outperform existing assertion schemes~\cite{zhou2019quantum,huang2019statistical} in terms of expressive power, flexibility, and efficiency.

\subsection{Quantum program logic and analysis with projections}

Projection operators have been used in logic systems and static analysis for quantum programs.
All projections in (the closed subspaces of) a Hilbert space form an orthomodular lattice~\cite{kalmbach1983orthomodular}, which is the foundation of the first Birkhoff-von Neumann quantum logic~\cite{birkhoff1936logic}.
After that, projections were employed to reason about~\cite{brunet2004dynamic} or develop a predicate transformer semantics~\cite{ying2010predicate} of quantum programs.
Recently, projections were also used in Hoare-like quantum logics for verification purposes~\cite{unruh2019quantum, zhou2019applied}.
Orthogonal to these prior works, this paper proposes to use projection-based predicates in assertion, targeting runtime testing rather than logic or static analysis.
\todo{}
% Unruh proposed quantum relational Hoare logic (qRHL) using subspaces as preconditions and postconditions~\cite{unruh2019quantum}. 


% More specifically, several static analysis tools have employed projections as predicates.

%\todo{}

%\subsection{Logical Reasoning about Quantum Programs}

%\myAssertionName~presents one more improvement over the previous work. The debugging schemes discussed above do not cooperate with a logic system and fail to derive the assertions automatically. But our scheme is based on a program logic, called aQHL (applied Quantum Hoare logic)~\cite{zhou2019applied}. Although it is a simplified version of quantum Hoare logic defined in~\cite{ying2010predicate}, aQHL is (relative) complete for projective assertions, which makes out our debugging scheme more powerful comparing with existing assertion schemes~\cite{zhou2019quantum,huang2019statistical}.



%\todo{}
%Note that all projections in (or, closed subspaces of) a Hilbert space form an orthomodular lattice \cite{KA83}, i.e. (the algebraic counterpart of) Birkhoff-von Neumann quantum logic \cite{BvN36}, and thus the power of quantum logic can be leveraged in reasoning about quantum programs. The first attempt of using quantum logic in reasoning about quantum programs was made in \cite{BJ04}.
%Projections were also employed in \cite{YDFJ09} to develop a predicate transformer semantics of quantum programs. However, no inference rules presented in this paper were derived in \cite{BJ04, YDFJ09}. 
%Several logic systems have been proposed to study quantum systems and programs.
%Birkhoff and von Neumann first studied the logic of quantum mechanics~\cite{birkhoff1936logic}, 
%Brunet and Jorrand first attempted to reason about quantum programs with logic~\cite{brunet2004dynamic}. 
%Ying \textit{et al.} developed a predicate transformer semantics with projections for quantum programs
%All these works do not have the inference rules that can be used for efficient debugging.

%Ying proposed Quantum Hoare Logic~(QHL)~\cite{ying2011floyd}, in which the predicates are general Hermitian operators.
%Although QHL can help derive correct formulas for quantum programs, it is not suitable for debugging schemes. 
%The reason is that when testing the correctness of a formula in QHL, a large number of destructive measurements are required to obtain an expectation of a Hermitian operator with enough accuracy, leading to time consuming debugging and testing.
%Although the expressive power of aQHL is strictly weaker than that o f
%This work employs applied Quantum Hoare Logic porposed by Zhou \textit{et al.}~\cite{zhou2019applied} and uses projective operators, a special class of Hermitian operators, as preconditions and postconditions to mitigate inefficient debugging.
%The expressive power loss in this restriction is not significant because the derivation of most existing algorithms is on pure states.
%of the correctness formulas.

%Unruh proposed quantum relational Hoare logic (qRHL) using subspaces as preconditions and postconditions~\cite{unruh2019quantum}. 
%The target of qRHL is to reason the equivalence of two quantum programs and verify quantum cryptography protocols. 
%By contrast, aQHL is tailored for debugging and testing, which provides simplified inference rules and can prove approximate satisfaction.

%Going further to the reactive system, Yu defined quantum temporal logic using projections in~\cite{yu2019quantum} and provided algorithms for basic logic formulae.


%\todo{Robust}
%Hung \textit{et al.} quantitatively analyzed the robustness of quantum programs and focused on reasoning about the behavior of faulty or noisy quantum programs~\cite{hung2019quantitative} rather than inexactly verifying quantum programs with error bounds.
%In this paper, we estimate the accumulated error of applying a series of assertions and show that the proposed debugging scheme is robust with small error.
%but qRHL aims at reasoning about equivalence between two quantum program (and targets applications in security verification of quantum cryptographic protocols) rather than correctness of quantum programs.





==> tex/9-Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

The demand for bug-free quantum programs calls for efficient and effective debugging scheme on quantum computers.
This paper enables assertion-based quantum program debugging by proposing \myAssertionName, a projection-based runtime assertion scheme.
In \myAssertionName, predicates in the \textbf{assert} primitives are projective operators, which significantly increase the expressive power compared with existing quantum assertion scheme.
%Cooperating with aQHL, in which the preconditions and postconditions are also projections, we can derive assertions at arbitrary place of a quantum program.
Several techniques are introduced to rotate the predicates to the computational basis, on which a realistic quantum computer usually supports its measurements, %so that a satisfying tested state will not be destroyed when an assertion is checked and multiple assertions per testing execution is enabled. 
so that the measurements in our assertions do not destroy the state when the assertion is satisfied.
Therefore, multiple assertions can be tested in one execution.
The superiority of \myAssertionName~is demonstrated by its applications to derive assertions for two well-known sophisticated quantum algorithms.
%\todo{Will change accordingly at the end}

%introduced a runtime assertion scheme for debugging on a quantum computer.
